Approximating Activation Functions

ReLU is widely seen as the default choice for activation functions in neural networks. However, there are cases where more complicated functions are required. In particular, recurrent neural networks (such as LSTMs) make extensive use of both hyperbolic tangent and sigmoid functions. These functions are expensive to compute. We used function approximation techniques to develop replacements for these functions and evaluated them empirically on three popular network configurations. We find safe approximations that yield a 10% to 37% improvement in training times on the CPU. These approximations were suitable for all cases we considered and we believe are appropriate replacements for all networks using these activation functions. We also develop ranged approximations which only apply in some cases due to restrictions on their input domain. Our ranged approximations yield a performance improvement of 20% to 53% in network training time. Our functions also match or considerably out perform the ad-hoc approximations used in Theano and the implementation of Word2Vec.

==> code/Theano-UltraFastSigmoid.tex <==

\definecolor{dkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}

\lstset{frame=tb,
  language=matlab,
  aboveskip=1mm,
  belowskip=1mm,
  showstringspaces=false,
  columns=flexible,
  basicstyle={\scriptsize\ttfamily},
  numbers=none,
  numberstyle=\scriptsize\color{gray},
  keywordstyle=\color{blue},
  commentstyle=\color{dkgreen},
  stringstyle=\color{mauve},
  breaklines=true,
  breakatwhitespace=true,
  tabsize=3,
  frame=single
}


\begin{figure}
    \caption{Julia Implementation of Theano's `ultra\_fast\_sigmoid` (non-optimised for reading).}
    \label{Theano-UltraFastSigmoid-Code}
    
    %
    \begin{center}
    \begin{tabular}{c}
    \begin{lstlisting}[linewidth=9.9cm]
function ultra_fast_sigmoid(x)
    x = 0.5 * x;
    if(x>=0) 
        z = ( x < 1.7 ? ( 1.5 * x / ( 1 + x ) ) : ( x < 3 ? (0.935409070603099 + 0.0458812946797165 * ( x - 1.7 ) ) : 0.99505475368673 ))  
    else
        xx = -x;
        z = -(xx<1.7 ? (1.5*xx/(1+xx)) :   (xx < 3 ? (0.935409070603099 + 0.0458812946797165 * ( xx - 1.7 ) ) : 0.99505475368673))
    end
    z = 0.5*( z + 1.0);
end
    \end{lstlisting}
    \end{tabular}
    \end{center}
    
    
\end{figure}

==> graphs/PercentageActivation_DemoNetwork.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,354.3999938964844); %set diagram left start at 0, and has height of 354.3999938964844

%Rounded Rect [id:dp967680853688335] 
\draw  [fill={rgb, 255:red, 130; green, 130; blue, 130 }  ,fill opacity=1 ] (70,118) .. controls (70,113.58) and (73.58,110) .. (78,110) -- (572,110) .. controls (576.42,110) and (580,113.58) .. (580,118) -- (580,142) .. controls (580,146.42) and (576.42,150) .. (572,150) -- (78,150) .. controls (73.58,150) and (70,146.42) .. (70,142) -- cycle ;
%Rounded Rect [id:dp38914135934312877] 
\draw  [fill={rgb, 255:red, 130; green, 130; blue, 130 }  ,fill opacity=1 ] (70,208) .. controls (70,203.58) and (73.58,200) .. (78,200) -- (572,200) .. controls (576.42,200) and (580,203.58) .. (580,208) -- (580,232) .. controls (580,236.42) and (576.42,240) .. (572,240) -- (78,240) .. controls (73.58,240) and (70,236.42) .. (70,232) -- cycle ;
%Straight Lines [id:da2830364007915982] 
\draw    (320,150) -- (320,198) ;
\draw [shift={(320,200)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da28038718813178276] 
\draw    (180,150) -- (180,198) ;
\draw [shift={(180,200)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da26354062789082033] 
\draw    (180,150) -- (189.61,198.04) ;
\draw [shift={(190,200)}, rotate = 258.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da5636220266963323] 
\draw    (180,150) -- (199.26,198.14) ;
\draw [shift={(200,200)}, rotate = 248.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da9788723183767005] 
\draw    (180,150) -- (170.39,198.04) ;
\draw [shift={(170,200)}, rotate = 281.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7506472811096048] 
\draw    (180,150) -- (160.74,198.14) ;
\draw [shift={(160,200)}, rotate = 291.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


%Straight Lines [id:da9693229847076665] 
\draw    (460,150) -- (460,198) ;
\draw [shift={(460,200)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da3834460747830828] 
\draw    (320,150) -- (320,198) ;
\draw [shift={(320,200)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da43619823400581237] 
\draw    (320,150) -- (329.61,198.04) ;
\draw [shift={(330,200)}, rotate = 258.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da4490776655546558] 
\draw    (320,150) -- (339.26,198.14) ;
\draw [shift={(340,200)}, rotate = 248.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da023931873722229824] 
\draw    (320,150) -- (310.39,198.04) ;
\draw [shift={(310,200)}, rotate = 281.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da9847461622244942] 
\draw    (320,150) -- (300.74,198.14) ;
\draw [shift={(300,200)}, rotate = 291.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


%Straight Lines [id:da3119559745445839] 
\draw    (460,150) -- (460,198) ;
\draw [shift={(460,200)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da9738070785969672] 
\draw    (460,150) -- (469.61,198.04) ;
\draw [shift={(470,200)}, rotate = 258.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da743500117564381] 
\draw    (460,150) -- (479.26,198.14) ;
\draw [shift={(480,200)}, rotate = 248.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da04148629937042325] 
\draw    (460,150) -- (450.39,198.04) ;
\draw [shift={(450,200)}, rotate = 281.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da5102174535078952] 
\draw    (460,150) -- (440.74,198.14) ;
\draw [shift={(440,200)}, rotate = 291.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


%Shape: Rectangle [id:dp15088497240088006] 
\draw  [fill={rgb, 255:red, 222; green, 222; blue, 222 }  ,fill opacity=1 ] (70,20) -- (580,20) -- (580,60) -- (70,60) -- cycle ;
%Straight Lines [id:da5984198074040563] 
\draw    (320,60) -- (320,108) ;
\draw [shift={(320,110)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da15783694307155116] 
\draw    (180,60) -- (180,108) ;
\draw [shift={(180,110)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7549169539625713] 
\draw    (180,60) -- (189.61,108.04) ;
\draw [shift={(190,110)}, rotate = 258.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da5894492267624181] 
\draw    (180,60) -- (199.26,108.14) ;
\draw [shift={(200,110)}, rotate = 248.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da5492611952219195] 
\draw    (180,60) -- (170.39,108.04) ;
\draw [shift={(170,110)}, rotate = 281.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da607802332325543] 
\draw    (180,60) -- (160.74,108.14) ;
\draw [shift={(160,110)}, rotate = 291.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


%Straight Lines [id:da8694444641431325] 
\draw    (460,60) -- (460,108) ;
\draw [shift={(460,110)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7675304893041535] 
\draw    (320,60) -- (320,108) ;
\draw [shift={(320,110)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da9101803677862315] 
\draw    (320,60) -- (329.61,108.04) ;
\draw [shift={(330,110)}, rotate = 258.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da366498641989381] 
\draw    (320,60) -- (339.26,108.14) ;
\draw [shift={(340,110)}, rotate = 248.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da6382833829659238] 
\draw    (320,60) -- (310.39,108.04) ;
\draw [shift={(310,110)}, rotate = 281.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da06574582232969117] 
\draw    (320,60) -- (300.74,108.14) ;
\draw [shift={(300,110)}, rotate = 291.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


%Straight Lines [id:da04717280377530275] 
\draw    (460,60) -- (460,108) ;
\draw [shift={(460,110)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da058498884816224006] 
\draw    (460,60) -- (469.61,108.04) ;
\draw [shift={(470,110)}, rotate = 258.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da5905241471607097] 
\draw    (460,60) -- (479.26,108.14) ;
\draw [shift={(480,110)}, rotate = 248.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da6279615429648826] 
\draw    (460,60) -- (450.39,108.04) ;
\draw [shift={(450,110)}, rotate = 281.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da020182037151676546] 
\draw    (460,60) -- (440.74,108.14) ;
\draw [shift={(440,110)}, rotate = 291.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


%Shape: Rectangle [id:dp1892014035286571] 
\draw  [fill={rgb, 255:red, 222; green, 222; blue, 222 }  ,fill opacity=1 ] (70,290) -- (580,290) -- (580,330) -- (70,330) -- cycle ;
%Straight Lines [id:da37308225327979483] 
\draw    (320,240) -- (320,288) ;
\draw [shift={(320,290)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8920407645887658] 
\draw    (180,240) -- (180,288) ;
\draw [shift={(180,290)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da9024704637841183] 
\draw    (180,240) -- (189.61,288.04) ;
\draw [shift={(190,290)}, rotate = 258.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da24344566325988093] 
\draw    (180,240) -- (199.26,288.14) ;
\draw [shift={(200,290)}, rotate = 248.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7609577307384046] 
\draw    (180,240) -- (170.39,288.04) ;
\draw [shift={(170,290)}, rotate = 281.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da3675941985685358] 
\draw    (180,240) -- (160.74,288.14) ;
\draw [shift={(160,290)}, rotate = 291.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


%Straight Lines [id:da6594451908125576] 
\draw    (460,240) -- (460,288) ;
\draw [shift={(460,290)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da526155096528766] 
\draw    (320,240) -- (320,288) ;
\draw [shift={(320,290)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da7800117383682561] 
\draw    (320,240) -- (329.61,288.04) ;
\draw [shift={(330,290)}, rotate = 258.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da8612486856985366] 
\draw    (320,240) -- (339.26,288.14) ;
\draw [shift={(340,290)}, rotate = 248.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da6803986681525549] 
\draw    (320,240) -- (310.39,288.04) ;
\draw [shift={(310,290)}, rotate = 281.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da6358414667536816] 
\draw    (320,240) -- (300.74,288.14) ;
\draw [shift={(300,290)}, rotate = 291.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


%Straight Lines [id:da16179240502084835] 
\draw    (460,240) -- (460,288) ;
\draw [shift={(460,290)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da3957695773292602] 
\draw    (460,240) -- (469.61,288.04) ;
\draw [shift={(470,290)}, rotate = 258.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da39733685997980106] 
\draw    (460,240) -- (479.26,288.14) ;
\draw [shift={(480,290)}, rotate = 248.2] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da883102641888359] 
\draw    (460,240) -- (450.39,288.04) ;
\draw [shift={(450,290)}, rotate = 281.31] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

%Straight Lines [id:da778831392886566] 
\draw    (460,240) -- (440.74,288.14) ;
\draw [shift={(440,290)}, rotate = 291.8] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;


%Shape: Brace [id:dp17132071265147397] 
\draw   (49,111.4) .. controls (44.33,111.4) and (42,113.73) .. (42,118.4) -- (42,165.4) .. controls (42,172.07) and (39.67,175.4) .. (35,175.4) .. controls (39.67,175.4) and (42,178.73) .. (42,185.4)(42,182.4) -- (42,232.4) .. controls (42,237.07) and (44.33,239.4) .. (49,239.4) ;

% Text Node
\draw (325,130) node  [align=left] {Dense (In = 28\textasciicircum 2, Out = 28\textasciicircum 2)};
% Text Node
\draw (325,220) node  [align=left] {Dense (In = 28\textasciicircum 2, Out = 28\textasciicircum 2)};
% Text Node
\draw (248.5,171) node  [align=left] {...};
% Text Node
\draw (391.5,171) node  [align=left] {...};
% Text Node
\draw (325,40) node  [align=left] {Input (n=28\textasciicircum 2)};
% Text Node
\draw (248.5,81) node  [align=left] {...};
% Text Node
\draw (391.5,81) node  [align=left] {...};
% Text Node
\draw (248.5,261) node  [align=left] {...};
% Text Node
\draw (391.5,261) node  [align=left] {...};
% Text Node
\draw (325,310) node  [align=left] {Output (n=28\textasciicircum 2)};
% Text Node
\draw (21,179.5) node [rotate=-270] [align=left] {Hidden Layers};


\end{tikzpicture}


==> graphs/PieChart.tex <==
\begin{tikzpicture}[scale=0.45][font=\tiny]
    \pie{ 29.36/Activation Time, 70.64/Other}
\end{tikzpicture}

==> maths/Approximate_Function_Implementation.tex <==
%https://varietyofsound.wordpress.com/2011/02/14/efficient-tanh-computation-using-lamberts-continued-fraction/
%\begin{figure}[]
%\caption{Definition of mathematical approximations.}
%\begin{equation}
%\label{Approximate-Maths-Function-Implementation}
%\begin{split}
%ReLU(x) &\approx ReLU(x)    = \frac{(x + |x|)}{2} \\
%exp(x)  &\approx exp(x,n)   =   %\prod_{1}^{\lg(n)}\big(1+\frac{x}{n}\big)^n\\
%tanh(x) &\approx tanh(x, n) = %\frac{x}{1+\frac{x^2}{3+\frac{x^2}{5+\dots}}}\\
%tanh(x) &\approx serpentine(a,b,x) = \frac{abx}{x^2 + a^2}
%\end{split}
%\end{equation}
%\end{figure}

%\renewcommand{\arraystretch}{2.5}


\begin{table}[]
\caption{Definitions of our chosen approximations. $B_n$ denotes the nth Bernoulli number.}
\centering
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Function}      & \textbf{Mathematical approximation}              & \textbf{Taylor}         & \textbf{Pad\'e}            \T\B \\\hline
$\mathrm{ReLU}(x) $    & ${(x + |x|)}*{0.5}$                              & N/A                     & N/A                        \T \\
$\tanh(x)$             & $\frac{x}{1+\frac{x^2}{3+\frac{x^2}{5+\dots}}}$  & $\sum_{i=1}^{n} \frac{2^{2i}(2^{2i}-1)B_{2i} x^{2i-1}}{(2i)!}$
                                                                                                    & TODO                       \T \\
$\text{sigmoid}(x)$    & $\frac{1}{1+\exp(-x)}$                           & N/A                     & N/A                        \T \\
$\exp(x)$              & $\prod_{1}^{\lg(n)}\big(1+\frac{x}{n}\big)^n$    & TODO                    & TODO                       \B \\\hline
\end{tabular}
\end{table}

==> maths/Function_Implementation.tex <==

%\begin{figure}[]
%\caption{Definitions of common activation functions.}
%\begin{align}
%\label{Maths-Function-Implementation}
%ReLU(x)    &= max(0, x) \\ 
%exp(x)     &= \lim_{n\to\infty}\Big(1 + \frac{x}{n}\Big)^n \\ 
%tanh(x)    &= \frac{ e^x - e^{-x} }{ e^x + e^{-x} } = \frac{ e^{2x} - 1 }{ e^{2x} + 1 } \\
%\end{align}
%
%\end{figure}



==> tables/ActivationFunctionCostTable.tex <==
\begin{table}
\centering
\caption{Costs of common activation function alongside the costs relative to ReLU running on an Intel i7-7700}
\label{Table-Activation-Function-Costs}
\begin{tabular}{|l|r|r|}
\hline
\textbf{Name}   & \textbf{Runtime ({$\mu$}seconds)} & \textbf{Relu Relative Time} \\ \hline
{ReLU~\cite{nair2010rectified}}          & 2.689                            & 1.000              \\ \hline
{SoftSign~\cite{bergstra2009quadratic}}      & 2.911                             & 1.082              \\ \hline
{LeakyReLU~\cite{maas2013rectifier}}     & 4.929                             & 1.833              \\ \hline
{ELU~\cite{clevert2015fast}}           & 9.600                             & 3.570              \\ \hline
\textbf{Sigmoid}& \textbf{9.801}                    & \textbf{3.645}     \\ \hline
{Swish~\cite{ramachandran2017searching}}         & 10.101                            & 3.757              \\ \hline
{SeLU~\cite{klambauer2017self}}          & 10.299                            & 3.830              \\ \hline
\textbf{Tanh}   & \textbf{21.300}                   & \textbf{7.921}     \\ \hline
{GeLU~\cite{hendrycks2016gaussian}}          & 25.200                            & 9.372              \\ \hline
{SoftPlus~\cite{glorot2011deep}}      & 33.099                            & 12.310             \\ \hline
{LogSigmoid}    & 42.201                            & 15.690             \\ \hline
\end{tabular}
\end{table}


%ORDERED 2000001 sample benchmark
%NNlib.σ: 29.354658500000003
%tanh: 58.234010999999995
%NNlib.relu: 10.6948235
%sigmoid_1: 11.1613125
%sigmoid_2: 12.413720999999999
%sigmoid_4: 11.739445
%sigmoid_8: 13.530307
%sigmoid_16: 12.8337025
%sigmoid_32: 13.0615425
%sigmoid_64: 13.884725
%sigmoid_128: 15.902431
%sigmoid_256: 15.453861999999999
%sigmoid_512: 16.254574
%sigmoid_1024: 17.4557815
%sigmoid_2048: 17.909755
%sigmoid_4096: 18.124795
%sigmoid_8192: 18.59683
%sigmoid_PolyLet7_Float64bit: 15.681702999999999
%sigmoid_PolyLet9_Float64bit: 16.26652
%sigmoid_PolyLet11_Float64bit: 16.124298
%sigmoid_PateLet33_Float64bit: 16.175783
%sigmoid_PateLet34_Float64bit: 17.157685
%sigmoid_PateLet44_Float64bit: 15.901292999999999
%sigmoid_PateLet45_Float64bit: 15.9893285
%sigmoid_PateLet55_Float64bit: 16.093577
%Serpentine: 10.527569999999999
%ApproxTanh6: 16.254573
%tanh_1: 11.75765
%tanh_2: 12.950752
%tanh_3: 12.808530000000001
%tanh_4: 13.945596499999999
%tanh_5: 15.5054895
%tanh_6: 16.988439500000002
%tanh_7: 18.497559499999998
%tanh_8: 19.434945
%tanh_9: 21.337310000000002
%tanh_PolyLet7_Float64bit: 16.112919
%tanh_PolyLet9_Float64bit: 16.036974
%tanh_PolyLet11_Float64bit: 16.583817500000002
%tanh_PateLet33_Float64bit: 16.5033195
%tanh_PateLet34_Float64bit: 16.691337500000003
%tanh_PateLet44_Float64bit: 16.2968135
%tanh_PateLet45_Float64bit: 16.4809905
%tanh_PateLet55_Float64bit: 16.993560000000002
%TheanoFastSigmoid: 13.77948%

==> tables/Sigmoid_Benchmark.tex <==
\begin{table}[]
\label{sigmoid-performance-data}
\caption{Relative run time costs of sigmoid approximations per 2 million calls.}
\begin{center}
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Function}                       & \textbf{Runtime (ms)}    & \textbf{\begin{tabular}[c]{@{}l@{}}Relative to\\ base sigmoid\end{tabular}} & \textbf{Average Error Per Input}             \\ \hline
\rowcolor[HTML]{EFEFEF} 
{\color[HTML]{000000} SigmoidPoly(7)}   & {\color[HTML]{000000} 15.68170} & {\color[HTML]{000000} 0.5342}                                               & {\color[HTML]{000000} 0.003464978658502659}  \\ \hline
\rowcolor[HTML]{EFEFEF} 
{\color[HTML]{000000} SigmoidPoly(9)}   & {\color[HTML]{000000} 16.26652} & {\color[HTML]{000000} 0.55413}                                               & {\color[HTML]{000000} 0.0012141550831330009} \\ \hline
\rowcolor[HTML]{EFEFEF} 
{\color[HTML]{000000} SigmoidPoly(11)}  & {\color[HTML]{000000} 16.124298} & {\color[HTML]{000000} 0.54929}                                               & {\color[HTML]{000000} 0.0003773057882240719} \\ \hline
\rowcolor[HTML]{C0C0C0} 
{\color[HTML]{000000} SigmoidPate(3,3)} & {\color[HTML]{000000} 16.175783} & {\color[HTML]{000000} 0.55104}                                               & {\color[HTML]{000000} 0.0005664979829501526} \\ \hline
\rowcolor[HTML]{C0C0C0} 
{\color[HTML]{000000} SigmoidPate(4,4)} & {\color[HTML]{000000} 15.90129299} & {\color[HTML]{000000} 0.54169}                                               & {\color[HTML]{000000} 1.86706721571719e-5}   \\ \hline
\rowcolor[HTML]{C0C0C0} 
{\color[HTML]{000000} SigmoidPate(5,5)} & {\color[HTML]{000000} 16.093577} & {\color[HTML]{000000} 0.54824}                                               & {\color[HTML]{000000} 3.533048494511567e-7}  \\ \hline
\rowcolor[HTML]{EFEFEF} 
Sigmoid(n=1)                            & 11.1613125                        & 0.38022                                                                      & 0.14133554553881394                          \\ \hline
\rowcolor[HTML]{EFEFEF} 
Sigmoid(n=32)                           & 13.0615425                       & 0.44495                                                                      & 0.0038474300624246095                        \\ \hline
\rowcolor[HTML]{EFEFEF} 
Sigmoid(n=128)                          & 15.902431                        & 0.54173                                                                      & 0.0009616729991928165                        \\ \hline
\rowcolor[HTML]{EFEFEF} 
Sigmoid(n=512)                          & 16.254574                        & 0.55373                                                                      & 0.00024041536056797704                       \\ \hline
\rowcolor[HTML]{EFEFEF} 
Sigmoid(n=4096)                         & 18.124795                        & 0.61744                                                                     & 3.0051896367040716e-5                        \\ \hline
\rowcolor[HTML]{C0C0C0} 
Theano:ultra\_fast\_sigmoid             & 13.77948                        & 0.46941     & 0.01293765234013063                          \\ \hline
\rowcolor[HTML]{C0C0C0} 
Word2Vec:Sigmoid w/lookup       & 324.01797100                        & 11.03804     & \textit{Variable}                          \\ \hline
\end{tabular}
\end{center}
\end{table}

%ORDERED 2000001 sample benchmark
%NNlib.σ: 29.354658500000003
%tanh: 58.234010999999995
%NNlib.relu: 10.6948235
%sigmoid_1: 11.1613125
%sigmoid_2: 12.413720999999999
%sigmoid_4: 11.739445
%sigmoid_8: 13.530307
%sigmoid_16: 12.8337025
%sigmoid_32: 13.0615425
%sigmoid_64: 13.884725
%sigmoid_128: 15.902431
%sigmoid_256: 15.453861999999999
%sigmoid_512: 16.254574
%sigmoid_1024: 17.4557815
%sigmoid_2048: 17.909755
%sigmoid_4096: 18.124795
%sigmoid_8192: 18.59683
%sigmoid_PolyLet7_Float64bit: 15.681702999999999
%sigmoid_PolyLet9_Float64bit: 16.26652
%sigmoid_PolyLet11_Float64bit: 16.124298
%sigmoid_PateLet33_Float64bit: 16.175783
%sigmoid_PateLet34_Float64bit: 17.157685
%sigmoid_PateLet44_Float64bit: 15.901292999999999
%sigmoid_PateLet45_Float64bit: 15.9893285
%sigmoid_PateLet55_Float64bit: 16.093577
%Serpentine: 10.527569999999999
%ApproxTanh6: 16.254573
%tanh_1: 11.75765
%tanh_2: 12.950752
%tanh_3: 12.808530000000001
%tanh_4: 13.945596499999999
%tanh_5: 15.5054895
%tanh_6: 16.988439500000002
%tanh_7: 18.497559499999998
%tanh_8: 19.434945
%tanh_9: 21.337310000000002
%tanh_PolyLet7_Float64bit: 16.112919
%tanh_PolyLet9_Float64bit: 16.036974
%tanh_PolyLet11_Float64bit: 16.583817500000002
%tanh_PateLet33_Float64bit: 16.5033195
%tanh_PateLet34_Float64bit: 16.691337500000003
%tanh_PateLet44_Float64bit: 16.2968135
%tanh_PateLet45_Float64bit: 16.4809905
%tanh_PateLet55_Float64bit: 16.993560000000002
%TheanoFastSigmoid: 13.77948

==> tables/TensorFlowResults.tex <==
%Swish time:58.2489369975196
%identity time:52.54747597376505
%NN Swish time:57.96209263801575
%NN Sigmoid time:55.606965939203896

\label{sigmoid-performance-data}
\begin{tabular}{|l|l|}
\hline
                       & \textbf{Runtime (s)} \\ \hline
\textbf{tf.nn.swish}   & 58.2489              \\ \hline
\textbf{tf.nn.sigmoid} & 55.6070              \\ \hline
\textbf{Identity}      & 51.2705              \\ \hline
\end{tabular}

